Distributed Deep Learning Using Volunteer Computing-Like Paradigm

Use of Deep Learning (DL) in commercial applications such as image classification, sentiment analysis and speech recognition is increasing. When training DL models with large number of parameters and/or large datasets, cost and speed of training can become prohibitive. Distributed DL training solutions that split a training job into subtasks and execute them over multiple nodes can decrease training time. However, the cost of current solutions, built predominantly for cluster computing systems, can still be an issue. In contrast to cluster computing systems, Volunteer Computing (VC) systems can lower the cost of computing, but applications running on VC systems have to handle fault tolerance, variable network latency and heterogeneity of compute nodes, and the current solutions are not designed to do so. We design a distributed solution that can run DL training on a VC system by using a data parallel approach. We implement a novel asynchronous SGD scheme called VC-ASGD suited for VC systems. In contrast to traditional VC systems that lower cost by using untrustworthy volunteer devices, we lower cost by leveraging preemptible computing instances on commercial cloud platforms. By using preemptible instances that require applications to be fault tolerant, we lower cost by 70-90% and improve data security.

==> arch.tex <==
\section{System Design} \label{sec:arch}
\begin{figure}
\centering
\includegraphics[scale=0.7]{./images/eydlearch}
 \caption{Architecture} \label{fig:arch}
\end{figure} \fxnote{Probably shud show server smaller in size?}

Figure \ref{fig:arch} shows the overall architecture of the Eydle system. In 
this section we will elaborate on the various individual components of Eydle.

We have built the Eydle distributed DL platform using the open source VC 
system, \textit{Berkeley Open Infrastructure for Network Computing} (BOINC). 
BOINC provides the base platform for creating a DL training application, that 
consists of a DL model server and a client that executes the DL model training 
jobs. The BOINC system provides its own client software within which the DL 
model training jobs are run.  \fxnote{Need BOINC citation here.} Additionally 
BOINC also has a job scheduler, a database to keep metadata about the 
application and its jobs. The application server and client communicate with 
each other over HTTP protocol using Apache2 server. The benefit of 
communicating over HTTP protocol is that no special ports need to be allowed 
for communication between DL server and client. This is especially 

